Zero-Shot Human-Object Interaction Synthesis with Multimodal Priors

Human-object interaction (HOI) synthesis is important for various applications, ranging from virtual reality to robotics. However, acquiring 3D HOI data is challenging due to its complexity and high cost, limiting existing methods to the narrow diversity of object types and interaction patterns in training datasets. This paper proposes a novel zero-shot HOI synthesis framework without relying on end-to-end training on currently limited 3D HOI datasets. The core idea of our method lies in leveraging extensive HOI knowledge from pre-trained Multimodal Models. Given a text description, our system first obtains temporally consistent 2D HOI image sequences using image or video generation models, which are then uplifted to 3D HOI milestones of human and object poses. We employ pre-trained human pose estimation models to extract human poses and introduce a generalizable category-level 6-DoF estimation method to obtain the object poses from 2D HOI images. Our estimation method is adaptive to various object templates obtained from text-to-3D models or online retrieval. A physics-based tracking of the 3D HOI kinematic milestone is further applied to refine both body motions and object poses, yielding more physically plausible HOI generation results. The experimental results demonstrate that our method is capable of generating open-vocabulary HOIs with physical realism and semantic diversity.

==> figures/part1_demo.tex <==
\begin{figure*}[tp]
    % \centering
    % \includegraphics[width=0.9\linewidth]{figures/part1_demo.pdf}
    % \includegraphics[width=0.75\linewidth]{figures/part1_demo.pdf}
    \includegraphics[width=1.0\linewidth]{figures/part1_results.jpg}
    \caption{part1 demo}
    % \Description{}
    \label{fig:part1_demo}
\end{figure*}

==> sections_v2/_preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% common preambles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%--------------------------------------------------
% colored text and comments
%--------------------------------------------------
\usepackage{bm}
\usepackage{bbm}
\newcommand{\blue}[1]{{\color{blue}{{#1}}}}
\newcommand{\libin}[1]{{\color{blue}{todo[libin]: {#1}}}}
\newcommand{\lbtmp}[1]{{\color{red}{{#1}}}}
\newcommand{\lb}[1]{{\color{blue}{{#1}}}}
\newcommand{\atl}[1]{{\color{teal}{{#1}}}}
\newcommand{\atltmp}[1]{{\color{magenta}{{#1}}}}
\newcommand{\revision}[1]{{\color{blue}{{#1}}}}

\renewcommand{\blue}[1]{{\color{black}{{#1}}}}
\renewcommand{\libin}[1]{{\color{black}{todo[libin]: {#1}}}}
\renewcommand{\lbtmp}[1]{{\color{black}{{#1}}}}
%\newcommand{\lb}[1]{{\color{black}{{#1}}}}
\renewcommand{\atl}[1]{{\color{black}{{#1}}}}
% \newcommand{\atltmp}[1]{{\color{black}{{#1}}}}
%\renewcommand{\revision}[1]{{\color{black}{{#1}}}}

%--------------------------------------------------
% for vectors (should be surrounded by $)
%--------------------------------------------------
\usepackage{graphicx}
\usepackage{tabularx}
\usepackage{subcaption}
\usepackage{multirow}
%\usepackage{gensymb}
\usepackage{amsmath}
%\usepackage{amssymb}
%\usepackage{mathtools}
\usepackage{mathrsfs}
\newcommand{\isep}{\mathrel{{.}\,{.}}\nobreak}
%\newcommand{\vect}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\vect}[1]{\bm{#1}}
\newcommand{\tildevect}[1]{\vect{\tilde{#1}}}
\newcommand{\hatevect}[1]{\vect{\hat{#1}}}
\newcommand{\unit}[1]{\widehat{#1}}
\newcommand{\sign}[1]{\operatorname{sign}(#1)}
\newcommand{\vecangle}[2]{(#1,#2)}
\newcommand{\eqword}[1]{{\text{#1}}}

%--------------------------------------------------
% common shortcuts in the text
%--------------------------------------------------
\usepackage{xspace}
\newcommand{\ie}{\textsl{i.e.}~}
\newcommand{\eg}{\textsl{e.g.}~}
\newcommand{\etal}{\textsl{et~al.}~}
\newcommand{\wrt}{\textsl{w.r.t.}~}
\newcommand{\NB}{\textsl{NB:}~}
\newcommand{\vs}{\textsl{vs.}~}
\newcommand{\cf}{\textsl{cf.}~}
\newcommand{\resp}{respectively\xspace}
\newcommand{\aka}{\textsl{a.k.a.}~}
\newcommand{\etc}{\textsl{etc.}}


%--------------------------------------------------
% Commands for keeping text (it's in the latex
%  but not displayed on pdf)
%--------------------------------------------------
\newcommand{\keep}[1]{}
\newcommand{\old}[1]{}

%--------------------------------------------------
% Math operators
%--------------------------------------------------
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\mse}{mse}
\DeclareMathOperator*{\simloss}{sim}
\DeclareMathOperator*{\stopgrad}{sg}
\DeclareMathOperator*{\softmax}{softmax}
\newcommand{\norm}[1]{\lVert #1 \rVert}

%--------------------------------------------------
% References
%--------------------------------------------------
\usepackage{url}
\usepackage{hyperref}
% \usepackage{refcheck}
\newcommand{\fig}{Figure{}~}
\newcommand{\eqn}{Equation{}~}

%\captionsetup[figure]{singlelinecheck=off}
%\captionsetup[subfigure]{singlelinecheck=off}
%\captionsetup[table]{singlelinecheck=off}

%--------------------------------------------------
% Symboles
%--------------------------------------------------
% the generator state
\newcommand{\vrc}{\ensuremath{{\bm{o}}}}



\usepackage[table]{xcolor} % for cell coloring
\usepackage{amssymb} % for checkmark and xmark
\usepackage{dingbat}
% Define custom colors for use in the table
\definecolor{checkcolor}{RGB}{0,128,0}
\definecolor{headercolor}{RGB}{0,0,0}
\definecolor{lightgray}{RGB}{224,224,224}

% Define commands for checkmark and xmark with colors
\newcommand{\cmark}{\textcolor{checkcolor}{\checkmark}}
\newcommand{\xmark}{\textcolor{red}{\sffamily X}}

==> sections_v2/_template_args.tex <==

%% NOTE that a single column version may be required for 
%% submission and peer review. This can be done by changing
%% the \doucmentclass[...]{acmart} in this template to 
%% \documentclass[manuscript,screen]{acmart}
%% 
%% To ensure 100% compatibility, please check the white list of
%% approved LaTeX packages to be used with the Master Article Template at
%% https://www.acm.org/publications/taps/whitelist-of-latex-packages 
%% before creating your document. The white list page provides 
%% information on how to submit additional LaTeX packages for 
%% review and adoption.
%% Fonts used in the template cannot be substituted; margin 
%% adjustments are not allowed.
%%
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
%\setcopyright{acmcopyright}
%\copyrightyear{2022}
%\acmYear{2022}
%\acmDOI{10.1145/1122445.1122456}
% \setcopyright{acmcopyright}
% \acmJournal{TOG}
% \acmYear{2022}
% \acmVolume{41}
% \acmNumber{6}
% \acmArticle{209}
% \acmMonth{12}
% \acmDOI{10.1145/3550454.3555435}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
\citestyle{acmauthoryear}
% \setcitestyle{square}

% A useful command for controlling the number of authors per row.
% The default value of "authorsperrow" is 2.
% \settopmatter{authorsperrow=4}

==> sections_v2/x_ack.tex <==

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
\begin{acks}
    We thank the anonymous reviewers for their constructive comments.
\end{acks}
    
